Hybrid lunar ISRU plant: a comparative analysis with carbothermal reduction and water extraction

To establish a self-sustained human presence in space and to explore deeper into the solar system, extensive research has been conducted on In-Situ Resource Utilization (ISRU) systems. Past studies have proposed and researched many technologies to produce oxygen from regolith, such as carbothermal reduction and water extraction from icy regolith, to utilize it for astronauts' life support and as the propellant of space systems. However, determining the most promising technology remains challenging due to uncertainties in the lunar environment and processing methods. To better understand the lunar environment and ISRU operations, it is crucial to gather more information. Motivated by this need for information gathering, this paper proposes a new ISRU plant architecture integrating carbothermal reduction of dry regolith and water extraction from icy regolith. Two different hybrid plant architectures integrating both technologies (1) in parallel and (2) in series are examined. The former involves mining and processing in both a Permanently Shadowed Region (PSR) and a peak of eternal light in parallel, while the latter solely mines in a PSR. In this series hybrid architecture, the dry regolith tailings from water extraction are further processed by carbothermal reduction. This paper conducts a comparative analysis of the landed mass and required power of each plant architecture utilizing subsystem-level models. Furthermore, based on uncertain parameters such as resource content in regolith, the potential performance range of each plant was discovered through Monte Carlo simulations. The result indicates the benefit of the series hybrid architecture in terms of regolith excavation rate, while its mass cost seems the highest among the studied architectures.

==> 0_Abstract.tex <==
To establish a self-sustained human presence in space and to explore deeper into the solar system, extensive research has been conducted on In-Situ Resource Utilization (ISRU) systems. Past studies have proposed and researched many technologies to produce oxygen from regolith, such as carbothermal reduction and water extraction from icy regolith. However, determining the most promising technology remains challenging due to uncertainties in the lunar environment and processing methods. To better understand the lunar environment and ISRU operations, it is crucial to gather more information. Motivated by this need for information gathering, this paper proposes a new ISRU plant architecture integrating carbothermal reduction of dry regolith and water extraction from icy regolith. 
Two different hybrid plant architectures integrating both technologies (1) in parallel and (2) in series are examined. The former involves mining and processing in both a Permanently Shadowed Region (PSR) and a peak of eternal light in parallel, while the latter solely mines in a PSR. In this series hybrid architecture, the dry regolith tailings from water extraction are further processed by carbothermal reduction.
This paper conducts a comparative analysis of the landed mass and required power of each plant architecture utilizing subsystem-level models. Furthermore, based on uncertain parameters such as resource content in regolith, the potential performance range of each plant was discovered through Monte Carlo simulations. The result indicates the benefit of the series hybrid architecture in terms of regolith excavation rate as well as its mass cost.
% To establish a self-sustained human presence in space and to explore deeper into the solar system, extensive research has been conducted on In-Situ Resource Utilization (ISRU) systems. Past studies have proposed and researched many technologies to produce oxygen from regolith, such as carbothermal reduction and water extraction from icy regolith. However, determining the superior technology remains challenging due to uncertainties in the lunar environment and processing methods. To tackle this uncertainty, it is crucial to gather more information to better understand the lunar environment and ISRU operations. Motivated by this, this paper proposes a new ISRU plant architecture integrating both carbothermal reduction of dry regolith and water extraction from icy regolith. 
% \rev{Two types of hybrid plant architectures integrating both technologies (1) in parallel and (2) in series are examined. The former involves mining and processing in both a Permanently Shadowed Region (PSR) and a peak of eternal light in parallel, while the latter solely mines in a PSR. In this series hybrid architecture, the dry regolith tailings from water extraction are further processed by carbothermal reduction.}
% % Two types of hybrid plant architectures, namely Type A and Type B, are examined. Type A involves mining and processing in both a Permanently Shadowed Region (PSR) and a Peak of Eternal Light (PEL) in parallel, while  Type B solely mines in a PSR. In this Type B hybrid architecture, the dry regolith tailings from water extraction are further processed by carbothermal reduction. 
% This paper conducts a comparative analysis of the mass and power of each plant design using subsystem-level models developed. Furthermore, based on uncertain parameters such as resource content in regolith, the potential performance range of each plant was discovered through Monte Carlo simulations. The result indicates the benefit of \rev{the series hybrid} architecture in terms of regolith excavation rate.% Moreover, the power consumption difference between the examined architectures proves to be relatively small.

% examines three plant architectures: carbothermal reduction of dry regolith, water extraction from icy regolith, and a hybrid combination of both technologies. Building a pilot plant relying only on one oxygen extraction technology or the other potentially limits the performance of the full-scale plant since actual performance is difficult to predict until deployed on the Moon. The proposed hybrid plant helps gather more information on system performance and supports decision-makers to make more informed choices regarding the deployment of a full-scale plant in a subsequent phase. Preliminary multi-objective decision analysis shows the viability of the hybrid pilot plant to improve product yield by about 10\% and mass payback by about 5\% compared to a carbothermal reduction plant. Further analysis reveals water content significantly affects the system mass and power consumption of both water extraction and hybrid plant architectures, highlighting the importance of gaining more information about lunar water ice. A more extensive analysis incorporates power consumption as an additional objective, providing a more comprehensive view of ISRU plant deployment decisions.  
